Machine Learning-Guided Memory Optimization for DLRM Inference on Tiered Memory

Deep learning recommendation models (DLRMs) are widely used in industry, and their memory capacity requirements reach the terabyte scale. Tiered memory architectures provide a cost-effective solution but introduce challenges in embedding-vector placement due to complex embedding-access patterns. We propose RecMG, a machine learning (ML)-guided system for vector caching and prefetching on tiered memory. RecMG accurately predicts accesses to embedding vectors with long reuse distances or few reuses. The design of RecMG focuses on making ML feasible in the context of DLRM inference by addressing unique challenges in data labeling and navigating the search space for embedding-vector placement. By employing separate ML models for caching and prefetching, plus a novel differentiable loss function, RecMG narrows the prefetching search space and minimizes on-demand fetches. Compared to state-of-the-art temporal, spatial, and ML-based prefetchers, RecMG reduces on-demand fetches by 2.2x, 2.8x, and 1.5x, respectively. In industrial-scale DLRM inference scenarios, RecMG effectively reduces end-to-end DLRM inference time by up to 43%.

==> figures/model_training_time.tex <==


\begin{table}[!t]
\caption{Training time, model size, and accuracy for all datasets.}
\scriptsize
\vspace{-10pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|c|ccc|ccc|}
\hline
                                                                                        & \multicolumn{3}{c|}{\textbf{caching model}}                                                                                                                                    & \multicolumn{3}{c|}{\textbf{prefetch model}}                                                                                                                                                                               \\ \cline{2-7} 
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# lstm\\stack\end{tabular}} } & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}training \\ time \end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}model\\size \end{tabular}} } & \textbf{accuracy} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}training \\ time \end{tabular}}} & \multicolumn{1}{c|}{{\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}model  \\size\end{tabular}}}} & {\color[HTML]{333333} \textbf{accuracy}} \\ \hline
1                                                                                       & \multicolumn{1}{c|}{429}                                                                      & \multicolumn{1}{c|}{37055}                                                                       & X\%                   & \multicolumn{1}{c|}{765}                                                                      & \multicolumn{1}{c|}{38290}                                                                                           & Y\%                                        \\ \hline
2                                                                                       & \multicolumn{1}{c|}{603}                                                                      & \multicolumn{1}{c|}{45055}                                                                       & X\%                   & \multicolumn{1}{c|}{962}                                                                      & \multicolumn{1}{c|}{74290}                                                                                           & Y\%                                        \\ \hline
3                                                                                       & \multicolumn{1}{c|}{745}                                                                      & \multicolumn{1}{c|}{63055}                                                                       & X\%                   & \multicolumn{1}{c|}{1059}                                                                     & \multicolumn{1}{c|}{110290}                                                                                          & Y\%                                        \\ \hline
\end{tabular}

\label{tab:training_summary}
\vspace{-12pt}
\end{table}



\begin{comment}
    \begin{table}[!t]
\caption{Training time and model size for all datasets.}
\scriptsize
\vspace{-10pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{|c|cc|cc|}
\hline
                                                                                        & \multicolumn{2}{c|}{\textbf{caching model}}                                                                                                                                 & \multicolumn{2}{c|}{\textbf{prefetch model}}                                                                                                                                                       \\ \cline{2-5} 
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# lstm\\stack\end{tabular}} } & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}training \\ time (mins)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}model size\\ (\# of param)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}training \\ time (mins)\end{tabular}}} & {\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}model size\\ (\# of param)\end{tabular}}} \\ \hline
1                                                                                       & \multicolumn{1}{c|}{429}                                                                      & 37055                                                                       & \multicolumn{1}{c|}{765}                                                                      &  38290                                            \\ \hline
2                                                                                       & \multicolumn{1}{c|}{603}                                                                      & 45055                                                                       & \multicolumn{1}{c|}{962}                                                                      & 74290                                             \\ \hline
3                                                                                       & \multicolumn{1}{c|}{745}                                                                      & 63055                                                                       & \multicolumn{1}{c|}{1059}                                                                     & 110290                                             \\ \hline
\end{tabular}

\label{tab:training_summary}
\vspace{-12pt}
\end{table}
\end{comment}

\begin{comment}
    
\begin{table}[H]
   \caption{Example LaTeX Table with \texttt{\textbackslash multicolumn}} 
   \label{tab:example_multicolumn}
   \small
   \centering
   \begin{tabular}{lccccr}
   \toprule\toprule
   \textbf{Header 1} & \textbf{Header 2} & \textbf{Header 3} & \textbf{Header 4} \\ 
   \midrule
   \multicolumn{3}{c}{Multiple Column Entry} & Item 4 \\
   Item 1 & Item 2 & Item 3 & Item 4\\
   \bottomrule
   \end{tabular}
\end{table}

\end{comment}


==> figures/model_training_time_new.tex <==
\begin{comment}

\begin{table}[H]
   \caption{Training time, model size, and accuracy for all datasets.}
   \label{tab:training_summary}
   \small
   \centering
   \begin{tabular}{lcccccc}
   \toprule\toprule
   & \multicolumn{3}{c}{\textbf{Caching Model}} & \multicolumn{3}{c}{\textbf{Prefetch Model}} \\
   \cmidrule(r){2-4} \cmidrule(r){5-7}
   \textbf{\# LSTM Stack} & \textbf{Training Time} & \textbf{Model Size} & \textbf{Accuracy} & \textbf{Training Time} & \textbf{Model Size} & \textbf{Accuracy} \\ 
   \midrule
   1 & 429 mins & 37,055 & X\% & 765 mins & 38,290 & Y\% \\
   2 & 603 mins & 45,055 & X\% & 962 mins & 74,290 & Y\% \\
   3 & 745 mins & 63,055 & X\% & 1,059 mins & 110,290 & Y\% \\
   \bottomrule
   \end{tabular}
\end{table}
\end{comment}


\begin{table}[t]
   \caption{Training time, model size, and accuracy of using various number of LSTM stacks in \name.}
   \label{tab:training_summary}
   \small
   \centering
   \begin{tabular}{cccc}
   \toprule\toprule
   \multicolumn{4}{c}{\textbf{Caching Model}} \\
   \textbf{\# LSTM Stacks} & \textbf{\makecell{Training Time \\(mins)}} & \textbf{\makecell{Model Size \\(\# of param)}} & \textbf{Accuracy} \\ 
   \midrule
   1 & 429 & 37,055 & 80\% \\
   2 & 603 & 45,055 & 82\% \\
   3 & 745 & 63,055 & 83\% \\
   \end{tabular}
   
   %\vspace{2mm} % Adds some space between the two tables
   
   \begin{tabular}{cccc}
   \toprule\toprule
   \multicolumn{4}{c}{\textbf{Prefetch Model}} \\
   \textbf{\# LSTM Stacks} & \textbf{\makecell{Training Time \\(mins)}} & \textbf{\makecell{Model Size \\(\# of param)}} & \textbf{Accuracy} \\ 
   \midrule
   1 & 765 & 38,290 & 39\% \\
   2 & 962 & 74,290 & 50\% \\
   3 & 1,059 & 110,290 & 50\% \\
   \bottomrule
   \end{tabular}
\end{table}
\begin{comment}
\begin{table}[H]
   \caption{Training time, model size, and accuracy for all datasets.}
   \label{tab:training_summary}
   \small
   \centering
   \begin{tabular}{lcccccc}
   \toprule\toprule
   & \multicolumn{3}{c}{\textbf{Caching Model}} & \multicolumn{3}{c}{\textbf{Prefetch Model}} \\
   \cmidrule(r){2-4} \cmidrule(r){5-7}
   \textbf{\makecell{\# LSTM\\ Stack}} & \textbf{Training Time} & \textbf{Model Size} & \textbf{Accuracy} & \textbf{Training Time} & \textbf{Model Size} & \textbf{Accuracy} \\ 
   \midrule
   1 & 429 mins & 37,055 & X\% & 765 mins & 38,290 & Y\% \\
   2 & 603 mins & 45,055 & X\% & 962 mins & 74,290 & Y\% \\
   3 & 745 mins & 63,055 & X\% & 1,059 mins & 110,290 & Y\% \\
   \bottomrule
   \end{tabular}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[H]
   \caption{Training time, model size, and accuracy of using various number of LSTM stacks in \name.} 
   \label{tab:training_summary}
   \small
   \centering
   \begin{tabular}{lccc}
   \toprule\toprule
   \multicolumn{4}{c}{\textbf{Caching Model}} \\
   \midrule % Adds a line below "Caching Model"
   \textbf{\# LSTM Stack} & \textbf{Training Time (mins)} & \textbf{Model Size (\# of param)} & \textbf{Accuracy (\%)} \\ 
   \midrule
   1 & 429 & 37,055 & X\% \\
   2 & 603 & 45,055 & X\% \\
   3 & 745 & 63,055 & X\% \\
   \bottomrule
   \end{tabular}
   
   \vspace{5mm} % Adds some space between the two tables
   
   \begin{tabular}{lccc}
   \toprule\toprule
   \multicolumn{4}{c}{\textbf{Prefetch Model}} \\
   \midrule % Adds a line below "Prefetch Model"
   \textbf{\# LSTM Stack} & \textbf{Training Time (mins)} & \textbf{Model Size (\# of param)} & \textbf{Accuracy (\%)} \\ 
   \midrule
   1 & 765 & 38,290 & Y\% \\
   2 & 962 & 74,290 & Y\% \\
   3 & 1,059 & 110,290 & Y\% \\
   \bottomrule
   \end{tabular}
\end{table}
\end{comment}

==> figures/sota.tex <==
\begin{comment}
\begin{table}[!ht]
    \centering
    \caption{ Existing Models for HPC}
    \label{tab:existing_ml}
    \begin{tabular}{|l|l|l|}
    \hline
        Model & Need Labels & Task \\ \hline
        GDN & ~ & ~ \\ \hline
        Prodigy & ~ & ~\\ \hline
    \end{tabular}
\end{table}
\end{comment}


\begin{table}[H]
   \caption{State-of-the-art Prefetcher}  
   \label{tab:example_multirow}
   \small
   \centering
   \begin{tabular}{lccccr}
   % \begin{tabular}{p{1.3cm}p{2cm}p{1 cm}p{1.2cm}p{1.2cm}p{0cm}}
   \toprule\toprule
   \textbf{Task} &\textbf{\makecell{Existing\\Work}} 
   &  \textbf{\makecell{Labeled \\Free}} &  \textbf{\makecell{Production \\ Telemetery}} &\textbf{\makecell{Application \\ Agnostic}}  \\ 
   \midrule
   \multirow{3}{*}{\makecell{Anomaly\\ Detection}} & Prodigy~\cite{aksar2023prodigy} & \xmark & \xmark &\xmark \\
                                       & RAUD~\cite{} &  \xmark & \checkmark &\checkmark\\
                                       & xxx~\cite{} &  \xmark & \checkmark &\checkmark\\
                                       & \textbf{Our solution} &  \checkmark & \checkmark &\checkmark\\
   \bottomrule
     \midrule
    \multirow{3}{*}{\makecell{Node Status\\ Detection}} & Prodigy~\cite{aksar2023prodigy} & \xmark & \checkmark &\xmark \\
                                       & RAUD~\cite{} &  \xmark & \checkmark &\checkmark\\
                                       & xxx~\cite{} &  \xmark & \checkmark &\checkmark\\
   \bottomrule
   \end{tabular}
\end{table}
